CooperBench: Why Coding Agents Cannot be Your Teammates Yet

Resolving team conflicts requires not only task-specific competence, but also social intelligence to find common ground and build consensus. As AI agents increasingly collaborate on complex work, they must develop coordination capabilities to function as effective teammates. Yet we hypothesize that current agents lack these capabilities. To test this, we introduce CooperBench, a benchmark of over 600 collaborative coding tasks across 12 libraries in 4 programming languages. Each task assigns two agents different features that can be implemented independently but may conflict without proper coordination. Tasks are grounded in real open-source repositories with expert-written tests. Evaluating state-of-the-art coding agents, we observe the curse of coordination: agents achieve on average 30% lower success rates when working together compared to performing both tasks individually. This contrasts sharply with human teams, where adding teammates typically improves productivity. Our analysis reveals three key issues: (1) communication channels become jammed with vague, ill-timed, and inaccurate messages; (2) even with effective communication, agents deviate from their commitments; and (3) agents often hold incorrect expectations about others' plans and communication. Through large-scale simulation, we also observe rare but interesting emergent coordination behavior including role division, resource division, and negotiation. Our research presents a novel benchmark for collaborative coding and calls for a shift from pursuing individual agent capability to developing social intelligence.

==> sections/06-coordination_table.tex <==
\definecolor{info}{RGB}{220,235,255}
\definecolor{integ}{RGB}{255,235,220}
\definecolor{struct}{RGB}{220,255,220}
\definecolor{comm}{RGB}{245,220,245}

\newcommand{\emojiicon}[1]{%
  \raisebox{-0.05em}{\includegraphics[height=1.15em]{#1}}%
}

\newcommand{\rootcell}[3]{%
  \parbox[t]{0.23\textwidth}{%
    \raggedright%
    \hspace{0.6pt}\strut%
    \textbf{\emojiicon{#1}\,#2}\par%
    \if\relax\detokenize{#3}\relax\else
      {\scriptsize\textit{#3}}\par%
    \fi
    \strut%
  }%
}

\begin{table*}[t]
  \centering
  \small
  \caption{Coordination failure causes. Causes reflect distinct coordination capability gaps.}
  \label{tab:failure_causes}

  \begingroup
  \setlength{\tabcolsep}{4pt}
  \setlength{\extrarowheight}{1.5pt}
  \renewcommand{\arraystretch}{1.25}

  \begin{tabular}{
    @{\hspace{2pt}}
    >{\raggedright\arraybackslash}p{0.25\textwidth}
    >{\raggedright\arraybackslash\footnotesize}p{0.70\textwidth}
    >{\centering\arraybackslash}p{0.05\textwidth}
    @{}
  }
    \toprule
    \textbf{Cause} & \textbf{Definition} & \textbf{\%} \\
    \midrule
    \rowcolor{info}
    \rootcell{figs/emoji/1f50d.png}{Expectation}{} & Cases where one agent has clearly communicated what they are doing, but the other agent still treats the situation as if that work is not being done. This reflects a failure to model the state of the other agent's code changes and what that means for the system as a whole. & 62.9 \\
    \midrule
    \rowcolor{comm}
    \rootcell{figs/emoji/1f4e3.png}{Communication}{} & Breakdowns in using language to coordinate. This includes failures in information sharing and decision loops between agents, where agents do not effectively communicate their intentions, questions, or status updates. & 27.5 \\
    \midrule
    \rowcolor{integ}
    \rootcell{figs/emoji/1f9e9.png}{Commitment}{} & Cases where an agent is not doing the things they promised to do. This includes failures to establish or maintain verifiable integration contracts, where agents make commitments but do not follow through on them. & 9.6 \\
    \bottomrule
  \end{tabular}
  \endgroup
\end{table*}

\begin{table*}[t]
  \centering
  \small
  \caption{Taxonomy of coordination failure symptoms. Symptoms are how coordination failures surface in merged artifacts.}
  \label{tab:failure_taxonomy}

  \begingroup
  \setlength{\tabcolsep}{4pt}
  \setlength{\extrarowheight}{1.5pt}
  \renewcommand{\arraystretch}{1.25}

  \begin{tabular}{
    @{\hspace{2pt}}
    >{\raggedright\arraybackslash}p{0.20\textwidth}
    >{\raggedright\arraybackslash\footnotesize}p{0.70\textwidth}
    >{\centering\arraybackslash}p{0.06\textwidth}
    @{}
  }
    \toprule
    \textbf{Symptom} & \textbf{Meaning} & \textbf{\%} \\
    \midrule
    Work overlap & Both agents independently implement the same functionality, duplicating work and overwriting details. & 33.2 \\
    Divergent architecture & Incompatible design decisions lead to semantic loss even under a clean merge. & 29.7 \\
    Repetition & Verbose status messages add little new information and reduce signal. & 14.7 \\
    Unresponsiveness & Direct questions or requests are not answered, breaking the decision loop. & 8.7 \\
    Unverifiable claims & Agent asserts a change or interface decision without evidence the partner can check (no checkable commitment). & 4.3 \\
    Broken commitment & Confident completion claims create false shared context when the promised change is absent. & 3.7 \\
    Dependency access & Missing risk communication leaves agents unable to anticipate merged dependency interactions (e.g., circular imports). & 1.7 \\
    Placeholder misuse & An explicit integration contract exists but is applied differently than agreed. & 1.5 \\
    Parameter flow & Ambiguity about a changing interface leaves one agent implementing against an outdated contract. & 1.3 \\
    Timing dependency & Agents agree on order but fail to communicate an enforceable plan that preserves it after merge. & 1.1 \\
    \bottomrule
  \end{tabular}
  \endgroup
\end{table*}

